Multi-Modal Temporal Attention Models for Crop Mapping from Satellite Time Series

Optical and radar satellite time series are synergetic: optical images contain rich spectral information, while C-band radar captures useful geometrical information and is immune to cloud cover. Motivated by the recent success of temporal attention-based methods across multiple crop mapping tasks, we propose to investigate how these models can be adapted to operate on several modalities. We implement and evaluate multiple fusion schemes, including a novel approach and simple adjustments to the training procedure, significantly improving performance and efficiency with little added complexity. We show that most fusion schemes have advantages and drawbacks, making them relevant for specific settings. We then evaluate the benefit of multimodality across several tasks: parcel classification, pixel-based segmentation, and panoptic parcel segmentation. We show that by leveraging both optical and radar time series, multimodal temporal attention-based models can outmatch single-modality models in terms of performance and resilience to cloud cover. To conduct these experiments, we augment the PASTIS dataset with spatially aligned radar image time series. The resulting dataset, PASTIS-R, constitutes the first large-scale, multimodal, and open-access satellite time series dataset with semantic and instance annotations.

==> experiments_ols.tex <==


\begin{table}[]
    \caption{Parcel-based classification performance in terms of Overall Accuracy (OA) and mean class-wise Intersect over Union (mIoU).}
    \vspace{.2cm}
    \centering
    \begin{tabular}{lccclcc}
    %\toprule
      Method   & OA & mIoU & \phantom{a} & Method   & OA & mIoU \\\cmidrule{1-3}\cmidrule{5-7}
    S2 Only     &  91.7  &    73.3    && S2 + TempDrop     &     &      \\
    S1A Only     & 86.7   &   63.4    && S1A + TempDrop     &     &       \\
    S1D Only     &   86.5        &   63.0     &&  S1D + TempDrop     &     &       \\\cmidrule{1-3}\cmidrule{5-7}
    Early Fusion + Interpolation &  92.2  & 75.5      &&  Ours - S1A     & 92.3   &    75.8      \\
    Decision Fusion + Aux    &   91.9  &  75.0     && Ours - S1D    &  92.2  &   75.5     \\
    Ours    &   \textbf{92.4} &   \textbf{76.3 }        && Ours - TempDrop    &  92.3   & 75.6         \\
%\bottomrule         
    \end{tabular}
    \label{tab:exp_parcel}
\end{table}

\begin{table}[h]
    \caption{Other stuff (temporary) }
    \centering
    \begin{tabular}{lcc}
     Method   & OA & mIoU \\\midrule
     Decision without Aux   & 90.8 & 72.1 \\
     Decision + Aux + TempDrop & 91.9 & 75.4 \\
     Late Fusion & 91.3 & 73.1  \\
     Ours + Interpolation & 91.9 & 74.7 \\
    \end{tabular}
    \label{tab:my_label}
\end{table}




\begin{table}[h]
    \caption{Caption}
    \vspace{.2cm}
    \centering
    \begin{tabular}{lccccccc}
    \toprule
             & & \multicolumn{2}{c}{Semantic}& & \multicolumn{3}{c}{Panoptic} \\\cmidrule{3-4}\cmidrule{6-8}
    Method   &\phantom{a} & OA     & mIoU& \phantom{abc} & SQ & RQ & PQ \\\cmidrule{1-1}\cmidrule{3-4}\cmidrule{6-8}
    S2 Only   &&  82.4   &  59.8  && 76.8  & 46.8 & 38.4  \\
    S1A Only   &&  78.3   &  50.4  &&   &  &   \\
    Ours   &&  \textbf{ 82.6}  &  \textbf{61.5}  && 77.6  & 45.5 &  37.7 \\\bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}


==> methods_old.tex <==
%...................................................
\subsection{Segmentation architecture}
%...................................................
Segmentation tasks such as semantic or panoptic segmentation require a specific architecture from the simpler parcel classification problem. We integrate our fusion scheme into the recent U-Net with Temporal Attention Encoder (U-TAE)  \cite{garnot2021utae}, which generalize the L-TAE approach to learning multi-scale pixel features which can be used in turn for semantic or panoptic segmentation.
%
In this section, we drop the assumption that the patch covered by $X$ contains necessarily only one parcel. Our goal is to produce a set of feature maps at different resolutions.

\paragraph{U-TAE architecture.} The U-TAE architecture for encoding a single modality image time series follows a five-step procedure:
\begin{itemize}
    \item[(i)] \textbf{Spatial Encoding.} Compute for each image independently a set of feature maps of decreasing spatial resolution with a shared multi-stage convolutional encoder. The resulting maps are concatenated in temporal dimension into a sequence of feature maps for each resolution.
    \item[(ii)] \textbf{Temporal Encoding.} Run a L-TAE network with $G$ heads for each pixel of the lowest resolution sequence independently. This produces $G$ low-resolution temporal attention maps, encoding which acquisitions contain the most relevant information for each head.
    \item[(iii)] \textbf{Attention Up-sampling.} Up-sample the attention maps to the resolution of all feature maps up to full resolution using bilinear interpolation. Each resolution level now has $G$ temporal attention maps associating to all pixels of all acquisitions their importance in the time series.
    \item[(iv)] \textbf{Temporal Averaging.} Compute the temporal average of each pixel across the image time series using the temporal attention maps as weights. The attention of a given head attends to a dedicated group of channels defined in advance. This results in a single feature map for each resolution: the \emph{innermost map} and the \emph{skip connections}.
    \item[(v)] \textbf{Spatial Decoding.}  A convolutional decoder takes the resulting feature maps and combines them in a classic U-Net fashion to produce refined feature maps at all resolutions.
\end{itemize}
We also refer the reader to the \cite[Sec.~3.1]{garnot2021utae} for more details on the design choices of this algorithm.
%
The next paragraph explains how each of these five steps should be modified to accommodate multi-modal image time series.
The first two steps can be adapted straightforwardly in the same manner than explained in the previous section: we spatially encode all modalities independently and merge the resulting feature sequences at the innermost level.
However, the next steps require special attention. Indeed, while radar images contain precious and cloud-robust information for determining the content of parcels, their high noise levels make them ill-suited to derive high-resolution information.
For this reason, we add two mechanisms to help prevent unwanted noisy information corrupting the high resolution feature maps: resolution-specific modality gating (RSMG) and modality-specific temporal attention maps (MSTAM).

For simplicity's sake, the subsequent explanation and equations are given for a L-TAE with a single head $G=1$. The equations for an arbitrary number of heads can be found in our appendix.

\paragraph{Spatial Encoding.} In a similar fashion to the parcel classification approach, each modality $m$ has its own dedicated multi-stage convolutional encoder $\spatial\m$. Such network is composed of $L$ levels $\spatial^{m,1},\cdots,\spatial^{m,L}$ producing feature maps $e^{m,l}$ with $F\m_l$ channels and of resolution $H_l=H/2^l$ and $W_l=W/2^l$ for $l\in[1,L]$. The maps are computed in parallel \wrt modalities and time and sequentially \wrt resolution levels:
\begin{align}
    e^{m,l}_t = \spatial^{m,1} \left(e^{m,l-1}_t \right), \forall m \in [1,M],\, t \in [1,T_m],\, l \in [1,L]~,
\end{align}
with $e^{m,0}_t=X\m,t$. The resulting maps at each level are concatenated temporally into a set of temporal sequences of feature maps $e^{m,l}$ of size $T\m \times F\m_l \times H_l \times W_l$.

\paragraph{Temporal Encoding.} Each pixel $h,w \in [1, H_L] \times [1,W_L]$ of the innermost sequence of feature maps is associated with $M$ time series $e^{m,l}_{h,w}$ of shape $T\m \times F\m_l$ for each modality $m$. Similarly to the parcel classification approach, we merge the different time series of spatial features into a single one to be processed with a L-TAE network. 
This network produces a temporal sequence of \emph{key-query compatibility} for each pixel and each modality, which can be rearranged into $M$ compatibility maps $z^{m,L}$ of size $T_m \times H_L \times W_L$.

The compatibility maps are used to compute modality-specific attention masks for each pixels 
 $T^\star \times H_L \times W_L$ 

%This network produces a temporal attention mask for each pixel, which can be rearranged into a single temporal attention map $a^{L}$ of shape $T^\star \times H_L \times W_L$ and with values in $[0,1]$, with $T^\star=\sum_m T_m$. 

\paragraph{Methods Segmentation WIP}


\begin{align}
    e^{m,l} &= [\Enc_l^m(e^{m, l-1}_t)]_{t=0}^{T}\;\;\text{for}\;\; l \in [1, L]\\
    e^L &= \text{merge}^{(T)}\left\{ e^{m,L}\right\}_{m=0}^M \;, T^* = \sum_m T_m\\
    &z^{L,1}, \cdots, z^{L,G} = \LTAE(e^L)\;\text{, applied pixelwise.} \\
    &a^{L,1}, \cdots, a^{L,G} = \text{softmax}_{T^*}(z^{L,1}), \cdots, \text{softmax}_{T^*}(z^{L,G}) \\
    &f^{L} = \text{Conv}_{1 \times 1}^L\left(\left[\sum_{t=1}^{T^*}a^{L,g}_t \odot e^{L,g}_t\right]_{g=1}^G\right)~\\
    &a^{m,l,1}, \cdots, a^{m,l,G} = \text{softmax}_{T_m}(z^{l,1}), \cdots, \text{softmax}_{T_m}(z^{l,G}) \\
    &a^{m,l,g} = \text{resize}\; a^{m,L,g} \;\text{to} \; H_l \times W_l\\
    &f^{l} = \sum_m \alpha_{m,l} * \text{Conv}_{1 \times 1}^{m,l}\left(\left[\sum_{t=1}^{T_m}a^{m,l,g}_t \odot e^{m,l,g}_t\right]_{g=1}^G\right)~\\
    d^{l}  &= \Dec_l([ \Dec^{\text{up}}_l(d^{l+1}), f^{l}]) \;\text{for}\; l \in [1, L-1]\\
\end{align}


\paragraph{Attention Up-sampling.}

start from sota architecture U-TAE , also based on l-TAE in a U-Net like architecture. 

